Multi-agent Application System in Office Collaboration Scenarios

This paper introduces a multi-agent application system designed to enhance office collaboration efficiency and work quality. The system integrates artificial intelligence, machine learning, and natural language processing technologies, achieving functionalities such as task allocation, progress monitoring, and information sharing. The agents within the system are capable of providing personalized collaboration support based on team members' needs and incorporate data analysis tools to improve decision-making quality. The paper also proposes an intelligent agent architecture that separates Plan and Solver, and through techniques such as multi-turn query rewriting and business tool retrieval, it enhances the agent's multi-intent and multi-turn dialogue capabilities. Furthermore, the paper details the design of tools and multi-turn dialogue in the context of office collaboration scenarios, and validates the system's effectiveness through experiments and evaluations. Ultimately, the system has demonstrated outstanding performance in real business applications, particularly in query understanding, task planning, and tool calling. Looking forward, the system is expected to play a more significant role in addressing complex interaction issues within dynamic environments and large-scale multi-agent systems.

==> table/03-office-tool-details.tex <==
\begin{table*}[t!]
\begin{tabular}{c c c p}
\toprule
\textbf{Scenario} & \textbf{API} & \textbf{Number of Parameters} & \textbf{Function Description} \\
\midrule
 & search\_email & 11 & Email search tool that helps users find emails based on input criteria such as start time, end time, etc. \\
Email & send\_email & 5 & Email sending tool that helps users send emails to specified recipients based on input such as email subject and recipient list. \\
 & summary\_email & 2 & Email summarization tool that generates text summaries based on a list of email IDs or the content of the current email. \\
\midrule
Schedule & create\_schedule & 5 & Schedule or meeting creation tool that helps users book schedules or meetings based on input such as subject, start time, and end time. \\
Schedule & update\_schedule & 7 & Schedule (including meetings) modification tool that helps users update schedules or meetings based on input information. \\
Schedule & find\_schedule\_status & 3 & Tool to check personal schedule or participant availability. It helps users determine if participants are free during a specified time range based on input such as participant list, start time, and end time. \\
Schedule & delete\_schedule & 1 & Schedule (meeting) deletion tool that helps users cancel schedules or meetings based on input information. \\
\midrule
Meeting & create\_meeting & 5 & Meeting creation tool, implemented by calling create\_schedule. \\
Meeting & find\_meetings & 2 & Meeting list search tool that helps users find related meetings based on input such as start and end time. \\
Meeting & find\_meeting\_room & 5 & Meeting room search tool that helps users find meeting room information based on input such as city, keywords, start time, and end time. \\
\midrule
Chat & search\_chatmsg & 7 & Chat message search tool that retrieves chat content based on input such as keywords, chat participants, and group names. \\
Chat & send\_chatmsg & 3 & Chat message sending tool that allows users to send messages and @mention specific people. \\
Chat & withdraw\_chatmsg & 2 & Chat message withdrawal tool that helps users withdraw specific chat messages based on input such as chat session ID (optional) and message ID. \\
Chat & summary\_chatmsg & 1 & Chat message summarization tool that generates summaries or abstracts based on a list of chat message IDs. \\
Chat & search\_group\_chat & 1 & Group chat search tool that searches for group chat names based on keywords. \\
Chat & find\_recent\_chat\_list & 2 & Chat session list viewing tool that searches for session lists based on time conditions. \\
\midrule
To-Do & create\_todo & 2 & To-do creation tool that helps users create to-do items based on input such as content and time. \\
To-Do & find\_todo & 3 & Tool to list personal to-do items, allowing users to query and filter their to-dos based on specified time and completion status. \\
To-Do & delete\_todo & 1 & To-do deletion tool that allows users to delete specified to-do items based on a list of to-do IDs. \\
\midrule
Cloud Document & search\_files & 13 & Cloud file search tool that supports file search and query based on user input with various filtering options. \\
Cloud Document & summary\_files & 1 & Cloud document summarization tool that generates summaries or abstracts based on a list of cloud document IDs. \\
\bottomrule
\end{tabular}
\caption{The statistics of our synthetic dataset in our \textit{specialized action distillation} method.}
\label{tab:tool-details}
\end{table*}

